BERGEN: A Benchmarking Library for Retrieval-Augmented Generation

Retrieval-Augmented Generation allows to enhance Large Language Models with external knowledge. In response to the recent popularity of generative LLMs, many RAG approaches have been proposed, which involve an intricate number of different configurations such as evaluation datasets, collections, metrics, retrievers, and LLMs. Inconsistent benchmarking poses a major challenge in comparing approaches and understanding the impact of each component in the pipeline. In this work, we study best practices that lay the groundwork for a systematic evaluation of RAG and present BERGEN, an end-to-end library for reproducible research standardizing RAG experiments. In an extensive study focusing on QA, we benchmark different state-of-the-art retrievers, rerankers, and LLMs. Additionally, we analyze existing RAG metrics and datasets. Our open-source library BERGEN is available under \url{https://github.com/naver/bergen}.

==> notes.tex <==
RQ 4. table 

remove bad dataets and take average 


 Stephane 

bm25 and golden at different positions

or change order of position 



different number of rand docs at random positions 

Thibault bm25 + reranker 
dense + reranker


David: new plots for 2,3 

Datasets exclude: 


Eli5, wow, sci, wikiqA, truthful QA

best datasets ASQA

FT asqa
